Photometric Redshift Uncertainties in Weak Gravitational Lensing Shear Analysis: Models and Marginalization

Recovering credible cosmological parameter constraints in a weak lensing shear analysis requires an accurate model that can be used to marginalize over nuisance parameters describing potential sources of systematic uncertainty, such as the uncertainties on the sample redshift distribution $n(z)$. Due to the challenge of running Markov Chain Monte-Carlo (MCMC) in the high dimensional parameter spaces in which the $n(z)$ uncertainties may be parameterized, it is common practice to simplify the $n(z)$ parameterization or combine MCMC chains that each have a fixed $n(z)$ resampled from the $n(z)$ uncertainties. In this work, we propose a statistically-principled Bayesian resampling approach for marginalizing over the $n(z)$ uncertainty using multiple MCMC chains. We self-consistently compare the new method to existing ones from the literature in the context of a forecasted cosmic shear analysis for the HSC three-year shape catalog, and find that these methods recover similar cosmological parameter constraints, implying that using the most computationally efficient of the approaches is appropriate. However, we find that for datasets with the constraining power of the full HSC survey dataset (and, by implication, those upcoming surveys with even tighter constraints), the choice of method for marginalizing over $n(z)$ uncertainty among the several methods from the literature may significantly impact the statistical uncertainties on cosmological parameters, and a careful model selection is needed to ensure credible parameter intervals.

==> processed_comments.tex <==
% \subsection{Photo-Z Uncertainty Models}
% \label{sec:mtd:models}

% In this section, we describe the models to describe the uncertainties of the photo-z sample redshift distribution $n(z)$ in this work. The models are probability distributions with increasing complexities. In Section~\ref{sec:mtd:shift}, we describe a simpler model that shift $n(z)$ around its mean values. In Section~\ref{sec:mtd:outlier}, we describe a more complex method that model the $n(z)$ as Gaussian Mixture Models (GMM) with an outlier rate. In Section~\ref{sec:mtd:cc}, we describe a model that use Dirichlet distributions to describe the histogram bin height of $n(z)$, with prior measured by cross correlating photometric and spectroscopic datasets. 

% \tianqing{Need to introduce the concept of `fiducial n(z)', which is an average of the cross correlation probability. This is later used to generate mock data vector.}

% \subsubsection{Additive and Multiplicative Shifting}
% \label{sec:mtd:shift}

% \subsubsection{Gaussian + Outlier}
% \label{sec:mtd:outlier}

% \subsubsection{Cross Correlation}
% \label{sec:mtd:cc}

% \rachel{`Cross Correlation' is about how you got the $n(z)$, rather than about the parametrization used.  I suggest calling it `Binned histogram with uncertainties on bin heights' or something like that.}



% \tianqing{Introduction should includes
% \begin{itemize}
%     \item Previous work of weak lensing shear and its cosmology implication.
%     \item Photo-Z and why sample redshift distribution is important in weak lensing analysis.
%     \item Previous work of $p(z)$ and $n(z)$ estimation.
%     \item Previous work on $n(z)$ error estimation.
%     \item Previous work of $n(z)$ error modeling in shear analysis.
%     \item State the purpose of this work: explore the appropriate $n(z)$ uncertainty modeling and marginalization method, in terms of variance-bias tradeoff.
% \end{itemize}
% }

%\rachel{My 2 cents: The above sounds very good (especially the concise summary of purpose).  The only small modification I suggest is that you should be as brief as possible on $p(z)$ estimation (individual objects), and focus primarily on the $n(z)$ estimation for the entire sample.  Otherwise this will be too long and might give the wrong impression about what is our concern.}





% \tianqing{Specification of this test:
% \begin{itemize}
%     \item Free parameter: $\Omega_m$ and $A_S$
%     \item $n(z)$ model: cross correlation model
%     \item Marginalization: resampling 50 $n_i(z)$ from $P(n(z))$, and combine with(out) Bayesian evidence
%     \item Covariance: $\mathbf{Cov}$, $\mathbf{Cov}/10$, and $\mathbf{Cov}/100$
%     \item $n(z)$ is shown in Fig.~\ref{fig:nz_cc}.
%     \item The MAP and 1-d contour of the 50 chains (with $\mathbf{Cov}$) in Fig.~\ref{fig:50chains}.
%     \item Results after marginalization in Fig.~\ref{fig:2params}.
% \end{itemize}}



% \tianqing{Specification of this test:
% \begin{itemize}
%     \item Free parameter:  $A_S$, $\Omega_b$, $n_s$, $h_0$, $\Omega_m$, $A_{IA}$, $\alpha$.
%     \item $n(z)$ model: cross correlation model
%     \item Marginalization: resampling 50 $n_i(z)$ from $P(n(z))$, and combine with(out) Bayesian evidence
%     \item Covariance: $\mathbf{Cov}$, $\mathbf{Cov}/10$, and $\mathbf{Cov}/100$
%     \item Contours shown in Fig.~\ref{fig:7params}.
% \end{itemize}}




% \begin{figure*}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{plot/7params_reg_cov.pdf}
%     \includegraphics[width=1.0\columnwidth]{plot/7params_medium_cov.pdf}
%     \caption{$2-\sigma$ contours on the $\Omega_m$-$\sigma_8$ plane and their 1-d posterior with 7 free parameters. The left chains use the original HSC Y1 covariance matrix $\mathbf{Cov}$, while the right plot use the $\mathbf{Cov}/10$. The resampling of the $n(z)$ will widen the parameter constraints in all cases. Using the Bayesian evidence as weights, the constraints are smaller than those that do not. Unsurprisingly, the $n(z)$ resampling has more impact on the medium covariance than on the regular covariance.  }
%     \label{fig:7params}
% \end{figure*}



% \tianqing{Specification of this test:
% \begin{itemize}
%     \item Free parameter:  $A_S$, $\Omega_b$, $n_s$, $h_0$, $\Omega_m$, $A_{IA}$, $\alpha$.
%     \item $n(z)$ model: $n(z) = \Bar{n}(z-\Delta z)$, fiducial values and prior listed in Table.
%     \item Marginalization: Run MCMC with 4 more $\Delta z_i$ parameter, total number of parameters: 11.
%     \item Covariance: I will start with $\mathbf{Cov}/10$.
%     \item The summary statistics in Fig.~\ref{fig:shift_summary}.
% \end{itemize}}







%\rachel{This was a key subsection, but it is quite long and complicated.  I recommend putting a single final subsubsection summarizing the list of methods either in a table or a bulleted list, indicating what abbreviation/label you will use for them in all plots and reminding the reader how many free parameters they have vs how many chains they need.  (I mean: in some case the uncertainty is included by adding some parameters, and in others it is by running multiple chains with different realizations.)  This is also a chance to introduce the trivial method you haven't talked about yet (no marginalization)!} \tianqing{Yeah, I have added a summary section.}

%\rachel{Side note, on the figure legends, I recommend changing all instances of `n(z) No Uncertainty' to `No n(z) Uncertainty'}


    \item \text{Fisher-PCA}: The $n(z)$ uncertainties of the bins are transformed into an orthonormal basis, where the covariance matrix of the uncertainties is an identity matrix. Fisher modes that maximize the cosmological impact are then found by an unitary transformation of the orthonormal basis. We use 6 nuisance parameters in this method to marginalize over redshift uncertainties, as described in Section~\ref{sec:mtd:fisher_pca}.
    
    
    
    
    
    
    
    
%\rachel{Note: I have commented out the longer descriptions that were in bullet points, as they seemed too detailed for a high-level intro to the section.  In context, I think they are out of place here, as we read them and then have a lot of text about something else in 3.1.  If you want to keep them, I suggest moving them to the introduction to 3.2 (which would require modest rearrangement, but not much).}\tianqing{A short version of the newly-proposed methods here is definitely more appropriate. No need to keep this now since we have the summary section that serves similar purpose.} %:
%\begin{comment}
%\begin{itemize}
%    \item \textbf{Bayesian Resampling:} A resampling approach that combines the chain from different $n(z)$ weighting by the model evidence, introduced in Section~\ref{sec:mtd:resample}.
%    \item \textbf{Fisher-PCA parameterization:} A parameterization that performs a two-step compression to the $n(z)$ uncertainties, firstly considers the leading components of the uncertainties with principle component analysis (PCA), and further making linear combination of the PCA mode based on maximizing Fisher information. This method is described in Section~\ref{sec:mtd:fisher_pca}.
%\end{itemize}
%\end{comment}
%\rachel{I think it's worth giving context -- the first one is the most straightforward, statistically accurate formulation of the problem IMO.  (In contrast to the second, which is clearly an approximation to the full error treatment as your description makes clear.)}\done


%In Section~\ref{sec:mtd:fisher_pca}, we propose a new parameterization approach by a two-step compression on the $n(z)$ parameters, simultaneously considering the leading components of the uncertainties and their cosmological impact using the Fisher matrix.



%In the top row of Fig.~\ref{fig:2params-2d}, we show the 1-d projection and 2-d contours on the $\Omega_m$-$S_8$ plane for the case of no $n(z)$ uncertainty along with the four marginalization approaches. In the bottom row, we show the log-evidence $\log(Z)$ of the chains in the resampling approach. The direct resampling method (purple) does not consider the Bayesian weight, while the Bayesian resampling method (red) does. \rachel{It is really striking that you do not discuss these results at all -- there's nothing about (a) Y3 vs full, (b) accuracy of parameter recovery, (c) how well the uncertainties are recovered, etc.  As a rule if you present a plot you should give some lesson learned from it.  This is connected to some structural issues I've highlighted in section 4.2.1.} 

%\tianqing{Appendix II will show the plot comparing the n(z) uncertainties that each method effectively consider.}


%\rachel{This is not typically considered as part of the cosmological model.  I suggest keeping 3.1.1 as a description of the cosmological model, and put a new short subsubsection after it for the intrinsic alignments model.  Or, if you want to keep this in this subsection, you should change the subsubsection title and intro sentence to emphasize that this is about both cosmological and astrophysical models.  Similarly, in table 1, both the caption and table should reflect that only some of the parameters shown are cosmological -- change wording and put a horizontal line to split cosmological and IA params.}\tianqing{Fixed. This is now a separate subsubsection. The table are divided too: one for cosmology parameters, one for astrophysical and nuisance parameters. } 
%\rachel{Different authors/surveys use different formulations of NLA, some with/without luminosity evolution, and with different signals.  For clarity, therefore, I think it is important to explicitly define the two parameters, i.e., to say how the effective IA amplitude for a given tomographic bin $i$ depends on $A$, $\eta$, and the redshift of bin $i$.  This would ideally be done with a single equation.} \tianqing{Done} \rachel{This is not how the model was formulated for HSC though -- for HSC, the $1+z_0$ in the denominator also had the power $\eta$ on it.  I'm not sure defining it with the power law only on the numerator makes sense.  Can you please check the code and confirm whether that was done?} \tianqing{Sorry, I put the parenthesis at the wrong place. Now it should be correct. }
%\rachel{Table and text use inconsistent notation ($A_\text{IA}$ versus $A$) -- should fix this and look for other places where it may be inconsistent.}\tianqing{Fixed.}


%\rachel{Note: this abstract previously referred to direct resampling and the shifting model without saying what those are.  I don't think we can reasonably do that (we have to define terms, and we don't have space to define them all), so I have changed it to refer to `existing methods in the literature.'  I also generalized the last sentence -- there are issues not only with overestimation but with underestimation, so I tried to make it more about the need for a principled choice. See what you think\dots} \tianqing{Yes, I like the ``statistically-principled Bayesian resampling'' versus the ``existing ones from the literature'', rather than causing confusion in the abstract by calling out their specific terminalogy. }


 %is the probability distribution of combining individual galaxy redshift probability $p(z)$ within a tomographic bin \ben{Reads slightly odd. "of the combined"? "of the combination of"? "of combining the"?}\tianqing{Improved the language here}. 
%% I commented the above discussion out because the reality is that there is no straightforward way to go from p(z) to n(z).  One has to combine them, deconvolve, and do many other complex processes -- the sentence was referring to a "combination" that sounded way too simple.

%\rachel{I think we should not only cite the Newman paper here.  That's a basic and purely frequentist presentation of the method.  In the meantime, Bayesian implementations have been developed and tested, e.g., in several of Markus's previous papers and some by DES folks such as Sanchez \& Bernstein.  We should acknowledge those importance contributions to this literature.}\tianqing{I have added Sanchez \& Bernstein and Rau et al. } \ben{Additionally, previous works aim to estimate $n(z)$ directly from photometric observables instead of relying on the photometric redshift~\citep[see, e.g.,][]{Lima_2008}, with the latter branching into machine learning and related approaches in recent years~\citep{Malz_2018, Henghes_2021}.}\tianqing{I have added this sentence to the text. }

%\rachel{this is a pretty random paper to specifically highlight  - why?  This was known for more than a decade before 2017.}\tianqing{Okay, I don't think we need to cite anything for this statement, yes?} 

%\rachel{We should consider whether to explicitly mention here that some recent analyses have not used $n(z)$ calibration methods that produce uncertainties in the needed form for resampling methods.}\tianqing{Sorry, can you elaborate which work is this? You mean they have no n(z) distribution to be sampled on?} \rachel{Yes, that is correct.  Example: the $n(z)$ derived by reweighting the COSMOS sample, as used for the HSC Y1 cosmic shear analyses.}\tianqing{OK. I think it is fine to ignore this here. But I have mention this in the drawbacks of the resampling methodology, in section 3.2.2.} 

% The "more recent" narrative doesn't work here, because the Hildebrandt paper is 2017, which is actually less recent than the papers cited above.

%\ben{The necessity of reliable $n(z)$ estimates for upcoming surveys is further discussed in~\citet{Malz_2022}.}\tianqing{Now have mentioned this in the first sentence of this paragraph.}

%We compare the resampling approach to the chains that parameterize $n(z)$ uncertainties as a shifting model. We propose a new parameterization that maximizes Fisher information on the principle components of the $n(z)$ uncertainties. 

 %\ben{The prior sentence is a bit confusing. Maybe something like "[...] and cover the modeling and marginalization of redshift distribution uncertainties in previous shear analyses."?}\tianqing{Yeah, agreed, it is applied.}

%\rachel{Should probably provide a brief overview of the weak lensing shear observables and how the ensemble $n(z)$ goes into it before transitioning into the topic you flagged:} 
%\tianqing{Introduce how n(z) error is modeled and marginalized over in previous shear analysis, e.g., the bin-shifting parameterization. }



%\rachel{Can you remind the reader how you found the MAP?  Directly from the chains using some utility, or with some method to reduce the noise in the MAP, such as the one used in DES?}\tianqing{I get this MAP directly from the chain. I showed this plot for 2-parameters cases for a reason: the MAP estimated by the chain for {\em only 2 parameters} are pretty accurate. But when the dimensionality goes up, we have to use the \textsc{maxlike} estimator, just like what DES did. So it is fine for the 2-params case, but if we want this plot for the full analysis, we need to use the MAP estimator (\textsc{maxlike}).} 


%\rachel{I'm confused why $W(z)$ has no index.  I thought it's supposed to incorporate the redshift distribution for sample $i$ as per equations further down, so shouldn't it have an index here and elsewhere?  Also, from a dimensional perspective, I am pretty sure the argument of the Bessel function needs to be $k\chi$ (to get something dimensionless), not $k_\chi(z)$, which would have units of wavenumber.  Finally, $\chi$ has not been defined.}\tianqing{Yes, $W(z)$ should be $W^i(z)$, same goes for eq. 4. Sorry that $k\chi$ was a typo, I don't even know whay I wrote $k_\chi(z)$... Fixed  }


%\rachel{ref needed for CAMIRA; need to define jargon S16A}\done


%\rachel{reference needed!  unless you were to rephrase to something more like `Since the IA model explicitly depends on redshift' (which is obvious from how you've formulated your model, so no reference is needed)}\tianqing{This is what I meant, I have updated the sentence.}, therefore, it is important to jointly fit the IA parameters in the parameter inference. 
%\rachel{Why not describe it here?  It fits here thematically and you've already pointed to the table, so I don't really see a value in splitting this info off into a separate subsection which has a different topic.}\tianqing{Now shear data vector is a separate subsubsection.}





%\rachel{Not clear what this means: do we set it to zero, or set it to a fixed nonzero value?  Regardless of what it means, I suggest putting it into table 1 for completeness, just like you've put some parameters that you've fixed (e.g., $\tau$).}\tianqing{I tweak the sentense to make it less confusing, also add the parameter to the table.} 

%\rachel{What happened to PSF additive systematics?  There are some parameters for them in table 2, but they are not discussed here in the model.}\tianqing{Nah, I am actively avoiding PSF in this paper.} \tianqing{They are added underneath.}

%\rachel{`Similar' implies it is the same in some ways and different in others.  How does it differ?  If it's actually the same model, then we should just say it's the same.}\tianqing{Yeah they are the same model.} 


%\rachel{The rest of this subsubsection is not about the cosmological model at all.  I think you need a new subsubsection called `Cosmic shear likelihood analysis'}\tianqing{Yes, the section is completely rearranged, now separated into 4 subsubsection: cosmology model; astrophysical and nuisance parameters; cosmic shear data vector; sampler,likelihood and covariance matrices.}

%\rachel{Need to comment on what assumption we are making about increasing amount of data for lensing vs.\ fixed covariances for n(z), and how that should be interpreted.}\tianqing{I have commented at the end of Section~\ref{sec:mtd:2pt_like}.}


%\rachel{should check - I think HSC used this too, in which case it might be good to cite both, just to show you are using choices that are relevant to the survey for which you are doing the forecasting}\tianqing{Yeah, Hamana et al. also use 0.62.}  
%\rachel{Comment on the other choices in that table - multiplicative bias and $\alpha$ and $\beta$?} \done 


%\rachel{can't you simply write this as an equation with $i=j$ rather than putting it in words after?  i.e., $\xi^{ii}_\pm(\langle N_i(z) \rangle_i) \ne \langle \xi^{ii}_\pm(N_i(z) ) \rangle_i$?  I'm not sure your current notation works, because $\xi^{ij}$ depends not only on redshift distribution $i$ but also on redshift distribution $j$}\tianqing{Good point, changed.} 

%\rachel{should this say `varying the efficiency'?}\tianqing{Yes. My original language was a bit confusing, I have edited this.} %\rachel{I think we have to say what efficiency it was fixed to?}\done


%\rachel{Justify/explain this.}\tianqing{It is the default value for \textsc{MultiNest}.}

%\rachel{Need to acknowledge the significant limitations in this approximation!}\tianqing{I added two limitation to our estimation.} \rachel{The first limitation listed is not relevant because the catalogs we use are full survey depth.  The bigger issue is that the survey footprint changes considerably (becomes more contiguous) as time goes on, so survey edge effects become less important, and our naive area factor does not account for that.}\tianqing{OK, I replace the first one with the issue you point out, and improve the level of details in the second one.} 

%\rachel{Need to say in what: redshift, angular separation, \dots}\tianqing{I meant angular binning.} 

%\rachel{I think changes in scale cuts are likely to be as important as this.}\tianqing{Added.}


%The mock cosmic shear analysis conducted in this work is as follow: (a) HSC Y3 covariance matrix with

%\rachel{100x is not particularly realistic; I would articulate it as a way to explore tradeoffs as the statistical errors change, including the extremes (tiny statistical error, not necessarily realistic).}
% \rachel{here it's a superscript but in table 4 it's a subscript - should be consistent in the paper text (including other sections) vs tables}\tianqing{Notations are homogenized.} 

%\rachel{Before saying how the shift is implemented, you have to say what exactly is the distribution that you are shifting.}\tianqing{Fixed} 




%\rachel{I'm a bit torn about the value of the detailed sentences above about the different methods.  Maybe consider whether you can omit the details about 3.2.1-3.2.3.  However, one very important thing that is missing is a clear statement of {\em what information do you have about $n(z)$ and its uncertainties}, and in what form, since that determines what methods are possible and how are they implemented.  I'm suggesting the addition of a very basic and short paragraph clarifying that $n(z)$ is determined in histogram bins, and explaining how the $n(z)$ uncertainty is represented.}\tianqing{I have added a paragraph above to clarify this important information.}


%\rachel{Inconsistent notation: here you use $E[z]$ a few times, while the table caption uses $\langle z_i\rangle$ to represent the same quantity.}\tianqing{I have changed all instances to $\langle z_i \rangle$} \rachel{Good, but you should also standardize on terminology - e.g., the table says `mean redshift' and the text says `expectation value of redshift'.  Please review the text of the section to make the terminology consistent with the table.}\tianqing{Fixed.}
%\rachel{Should consider whether this can be briefer, because in a previous section you already defined these two covariances.  So perhaps you could just mention that you use the two covariances defined previously?}\tianqing{Yeah, I have refer to the previous section for the covariance matrices. } 
%In Section, we run two analyses using different covariance matrices, $\mt{\Sigma}_{y3}$ for the three-year HSC dataset and $\mt{\Sigma}_\text{full}$ for the full HSC dataset, previously defined in Section~\ref{sec:mtd:2pt_like}.  %\rachel{I think this notation is obscuring the meaning.  These are estimated covariance matrices for Y3 and a hypothetical future analysis with 10x the area of HSC Y1.  So I suggest that when you describe this methodology, define symbols $Cov_{Y3}$ and $Cov_\text{future}$ or something like that, and use them throughout.  The key point is that {\em you want the symbols to be meaningfully descriptive of the scenario}, whereas $\Sigma_{y3}$ is technically descriptive (you literally divide by 3) but doesn't necessarily convey why you would want to do this.} \tianqing{We have switched to $\mt{\Sigma}_{y3}$, and $\mt{\Sigma}_{\text{full}}$. I add a descriptive text here to elaborate the meaning of the notation again, though they are explained in Section~\ref{sec:mtd:2pt_like}}

%\rachel{As a side note, I don't think we should use math-mode partial words like $Cov$ -- I would suggest $\vect{C}$ or $\mt{\Sigma}$ for covariances.}\tianqing{Fixed.}


%\rachel{Below are some overall comments from my reading on the plane on Tuesday (it's possible some have been taken care of since then).}

%\rachel{Comments on consistency of notation, for which the paper needs a careful review:
%\begin{enumerate}
    %\item Sometimes we refer to the `shift' model and other times the `shifting' model in the text / tables / figure legends.  Should pick one name for it.
    %\tianqing{unify to `shift' model.}
    %\item Table 6 and the summary section 3.4.3 use different notation and terminology.  Once there is a terminology and notation table, it really needs to be used consistently through the entire paper.  Should fix 3.4.3 and look for other instances.
    %\tianqing{If you meant Table.~\ref{tab:terminology} vs. Sec.~\ref{sec:mtd:summary}, they are homogenized.}
    %\item Figure 3 axis label vs caption vs text vs equations use different ways of referring to the evidence and weights; should make them consistent.
    %\tianqing{Homogenized to log-evidence $\log(P(D|nz_s))$ and Bayesian weight $\omega_s$.}
    %\item While there have been some improvements, there are still inconsistencies in how scalars, vectors, and matrices are indicated (which may seem like a minor detail, but for those who are new to your notation, using consistent signaling for these different types of quantities can be helpful).  Example: the FoM equation implies that the Fisher matrix is a scalar.  I suggest reviewing the MNRAS author guide, which specifies `Scalar variables are italic; vectors are bold italic (no arrows); matrices are bold Univers font (like bold sans serif)' and then making the entire paper consistent with it.
   % \tianqing{I have defined the new commands `mt', and `ve' for the matrices and vector. And change the things I see to this standard. Like matrix $\mt{\Sigma}$, or vector $\ve{D}$, and scalar $N_{\text{tomo}}$.} \rachel{I'm looking at section 2 and it might need some additional review (I see some that don't use these commands).}
    %\item You use $i$ as histogram bin in section 2.2 but then it denotes tomographic bin in sections 2.1 and 3. Sometimes $j$ is histogram bin, e.g., in $n^i(z_j)$ and but then in section 2.1, $j$ is also used for tomographic  bin.  I suggest having some well-defined scheme such as $i$, $j$ are tomographic bins and $k$ is histogram bin, and then implement it throughout the entire paper.
    %\tianqing{Sure, let's reserve $i$ and $j$ for tomographic bins, use $k$ for histogram bin heights, use $s$ for resampling index. Let's set all tomographic index to superscipt, e.g., $\xi^{ij}$, $n^i(z)$. Let's set the others to subscripts. }
    %\item There are probably too many ways of referring to redshift distributions: $n(z)$ vs $n^i(z)$ (superscript) vs $n_i(z)$ (subscript in section 2.2) vs $n^i(z_j)$.  I understand you might want one way to refer to redshift distributions in general, $n(z)$, but then when you are specifying that it's for a tomographic bin you should pick one notation (subscript or superscript) and when you further want to indicate that it's specifically Markus's representation in histogram bins, you can use something that refers to the bin indices.  I suggest actually defining these notations explicitly and using them consistently.\tianqing{I have sweep the paper and change the notation to `$n(z)$ prior' when we are not specifying the tomographic bin, and `$n^i(z)$' when we do. Additionally, all indices related to tomographic bins are in the superscript. }
%\end{enumerate}}

%\rachel{Comments on choices of how to present the work:
%\begin{enumerate}
    %\item In section 4.1, you use the means of the posterior, while in section 4.2, you use the MAP. What is the motivation for these different choices?  It's not clear and it seems to me that we should be consistent (or at least explain why we aren't consistent). \tianqing{At a second thought, it is double-beneficial to change Fig.~\ref{fig:200chains} to mean. It help the consistency in two things: the consistency in summary statistics and consistency in showing the full analyses results.}
    %\item The reference to $1\sigma$ error in section 4.1 (regarding figure 4) is not clear to me.  Does that mean you literally took the standard deviation, which is equivalent to modeling the posterior as a Gaussian?  It's not clear to me that you want to do that - it might make more sense to show the 68\% confidence intervals. Do those two things differ in practice? Let's discuss. 
    %\tianqing{Both the 1-d errorbars and 2-d contours are $68\%$ confidence interval. So I have change all `1-$\sigma$' to `$68\%$ confidence interval'.}
    %\item In figure 4, I understand why you are using the `No n(z) uncertainty' case as a reference, but I think it's important to keep in mind that people normally use plots that look like this to assess both (a) what happens to errorbars when we change analysis choices and (b) what biases are induced when we change analysis choices.  Therefore, I think it's important to also put a vertical line at the true cosmological parameters (despite keeping the shaded region as is).  Otherwise people will be too tempted to use the current vertical line and shaded region to do both (a) and (b), and they will get the answer wrong for (b).  It will also make figures 3 versus 4 easier to understand consistently. \tianqing{Added the truth reference lines (this took much effort). Also commented briefly on why the mean value of $\Omega_m$ is shifted to the lower end on both the caption and the main text. }
    %\item You should consider whether some of your text is too specific to your analysis setup.  Example: you emphasize in a few places that the shift model introduces 4 extra parameters.  But that's only because you have 4 tomographic bins.  So you might want to introduce a parameter such as $N_\text{tomo}$ to represent the number of tomographic bins, and say that you have $N_\text{tomo}=4$ nuisance parameters.  This helps remind the reader that if they use a different number of tomographic bins in their analysis, this might work out a bit differently for them.
    %\tianqing{I agree. I have replaced a lot of the plain `[...] 4 nuisance parameters' with `[...] $N_{\rm tomo} = 4$ nuisance parameters'.}
    %\item I feel we might not be very clear on the assumptions behind our implementation of resampling.  Correct me if I'm wrong, but I think our choice to use the posterior from Markus's method as the prior for our resampling methods is assuming that {\em the information from Markus's method is largely independent of our data vector} -- i.e., we use the weak lensing data vector, while he has used photo-z and cross-correlation measurements, so they are independent and one can be used as the prior for the other.  That independence might not be true in all cases (example: if we had done 3x2pt using some of the same reference spectroscopic samples as our lenses) and so the assumption of independence should be called out, if I'm indeed correct that the assumption is there.
    %\tianqing{I think so. This is explicitly mentioned in the last paragraph of Section~\ref{sec:bgd:nz_estimation}: `{\em The aforementioned posteriors of sample redshift distributions constructed using the joint likelihood of spatial cross-correlations and photometry is then used as the prior distribution on the sample redshift distribution in the following analysis.}'.}
%\end{enumerate}}

%\rachel{Comments on content:
%\begin{enumerate}
   % \item Right now the abstract, intro, and other text (e.g., section 4.3 and the bullet points for the conclusion) emphasizes the final findings regarding the resampling techniques and the shift model.  I was wondering if it would also be valuable to emphasize that the paper illustrates methodology that others can/should use if they want to select a method of marginalizing over N(z) uncertainties?  In other words, both the journey and the destination are important.
  %  \tianqing{Add this comments in Section~\ref{sec:mtd:summary}: `{\em For cosmic shear analyses with a substantial uncertainties on the sample redshift distribution, we recommend comparing any candidate marginalization methods for $n(z)$ with the results from the Bayesian resampling method, as the Bayesian resampling method provide a statistically-principled posterior on the marginalized parameters. }'. I will add a further comments like this in the conclusion section. }
   % \item There does not seem to be any literature comparison.  I know we are doing this because there haven't been many principled tests of this issue, but surely some groups must have compared e.g., no marginalization vs their adopted marginalization method (e.g., we did this in the Hamana et al cosmic shear paper), and we can compare against those results?
    %\tianqing{I have written a literature comparison section in the results.}
%\end{enumerate}
%}



% Following the methodology developed in \citet{2022MNRAS.509.4886R} (todo: more references) the redshift $z$ of the galaxy is then connected with the SED model to yield the galaxies' flux $f$. Describing the measurement process using the flux likelihood $ p(\vect{f}_i | \mathcal{T}(z_i), \Sigma)$, where ($\mathcal{T}$, $\Sigma$) denotes the (template model, flux measurement covariance), we can obtain a log-likelihood as: 
% \begin{equation}
%     l(\vect{\hat{F}}|\vect{nz}) = \sum_{i = 1}^{N_{\rm _{gal}}} \log{\left( \int \mathrm{d}z_i p_{\rm i}(\vect{f}_i | \mathcal{T}(z_i), \Sigma_i) \,  p(z_i | \vect{nz})\right)} \, .
%     \label{eq:likelihood}
% \end{equation}

% The likelihoods for the individual methods are treated in a model combination scheme that specifies a joint prior over the parameters $\vect{nz}$, which we denote as $p(\vect{nz} | \boldsymbol{\alpha})$.

%  We therefore include model uncertainty in a hierarchical manner by using a joint distribution over the parameters $\vect{nz}$ parametrized by $\boldsymbol{\alpha}$. 



%\tianqing{Introduce in detail the photo-z sample redshift estimation methods, e.g., Markus's cross-correlation n(z). }

%\rachel{It is easy to confuse photometric redshift estimation (which traditionally refers to individual object estimates) versus the estimates of calibrated $n(z)$ for ensembles.  I suggest selecting section titles that avoid such confusion.  For example, 2.1 and 3.1 could be an issue.}


%\rachel{Should clarify whether this is a traditional Fisher matrix calculation using derivatives of data vectors, or whether you took the posterior from MCMC and approximated it as a Gaussian to get a covariance matrix then inverted to a Fisher matrix.  With removal of Fisher-PCA method, you haven't talked about Fisher matrices yet in this paper.  Also need to say whether this is with other parameters marginalized or fixed.}\tianqing{These issues are addressed.} 


%\rachel{One thing that generally confuses me:  In figure 4, the 1D posterior for $\Omega_m$ is always peaked to the left of the true value.  But in figure 5, the point (which is described as the max of the 1d posterior) is always right on the truth.  How is this possible?  The figures seem to imply inconsistent things about the 1d posteriors.}\tianqing{Yeah, this is pretty confusing. So the dashed line in the 2-d plots are the true inputs. However, the dashed lines in the 1-d plots are the mean of the ``No uncertainties'', and the point estimation quoted in the 1-d plots are also the mean values, not the MAP. So it is normal that they are not consistent. I have addressed this in the texts. } \rachel{OK - but see my comment on this at the front of the paper.}\tianqing{Yeah, we should use mean statistics entirely. }

%\rachel{variance usually implies a scatter; is that what you mean?  I thought these were noiseless.  If you mean there are systematic deviations that compensate (e.g., always low in some places and always high in others) then I think you should say that instead.  And does this hypothesis come from inspecting some of the mock data vectors and their best-fitting theory?}\tianqing{There are two possibilities: (1) the nz realization generate data vector that has the same best-fit $D$ as the mock data vector, but having more noise (like zig-zagging around the mock DV. (b) the best fit data vector for the nz realization is biased from the mock, but it is compensated by other parameters, so it does not show up in $\Omega_m-S_8$ plane.)}
%One possible explanation is that the theoretical data vector generated by some $nz_s$ can have the same best-fit value as the observed data vector, however with higher variance, thus having a lower overall evidence.

%\rachel{A few paragraphs ago, you commented on this same point and explained it in terms of banana-shaped contours, and did not give any comment on the MAP.  I don't think you should raise the same issue twice and explain it differently; just explain it once and then refer back to it.  So I suggest finding the first place you have commented on this and consolidating the explanation, then changing this and future mentions.} \done
%\rachel{Should comment on some of the low-weight instances near the truth.  Also should say explicitly in figure caption what the dashed lines are.}\tianqing{\quo{We notice that there are $nz_s$ samples that generate mean posterior at the centre of the cluster, however receiving a very low weight. Here is our explanation:[...]}}

%\rachel{Is there a particular reason we have to show this in the 2-parameter case and not the full case?  It seems striking (and maybe surprising) that we show most of the lessons in the previous subsection but then this one is here.}\tianqing{Remember the MAP in the high dimensional cases suffers from the instability? To do this in full analyses, we need to run other MAP-estimator such as \textsc{MaxLike}. These MAP-estimator are convex optimizers, they heavily rely on the starting point, so we need to carefully tune them if we want to use them. } \tianqing{Since you've suggested that we use mean posterior as the summary statistics throughout, it is totally possible to do this for full analyses.}

%\rachel{I think this should just be `shift model' - we only have one parameterization method at this point}\tianqing{Fixed, also searched for other places.}. \rachel{Why is the CPU time per chain longer for no $n(z)$ uncertainty than for the resampling approaches?  I thought they have the same number of parameters. It is striking that no $n(z)$ uncertainty is nearly identical to the shift model in this regard, and could not figure out why.  If it's because of the number of live points, that just begs the question of why different numbers were adopted here.}\tianqing{Yeah, the only difference is the number of live points. I lower the live points for the resampling to speed up the process.  }


% Note, "order-of-magnitude" should be hyphenated when it's an adjective, i.e., "an order-of-magnitude estimate", but not when it's a noun.



%\rachel{Since we've only said this now, it makes our previous endorsement of the shift model based on computational expense seem a bit premature.  Should rethink the order of these steps; perhaps the previous endorsement on that basis should be removed given that we say it again in the next paragraph.}\tianqing{Yes, this makes sense. I have clipped that statement here and slightly edit it.} 



%\subsection{Supporting results}
%\label{sec:res:comparison}

%In this section, we show supporting results that help us better compare the $n(z)$ marginalization methods. In section~\ref{sec:res:2p-exp}, we discuss the inference results with only two free cosmological parameters, i.e., $\Omega_m$ and $\sigma_8$. In section~\ref{sec:res:other}, we discuss the implication of our results versus the exploration in the $n(z)$ marginalization done in other work.

%\rachel{Structural issue: this is a subsubsection inside the full analysis section, but then you are talking about the two parameter case, which doesn't make sense.  I think you have two options: (1) talk about implications of the two-parameter results in the two-parameter result section, which makes a lot of sense to me.  (Right now, you show the plots and don't talk about their implications at all, so the section looks pretty incomplete.)  Or (2) make `Methods comparison' a subsection, rather than a subsubsection, to capture the method comparison for 2-parameter and full.  But I really want to advocate for option (1) -- talk about the 2-parameter results in 4.1 and the full analysis results in 4.2, so that you don't have to present results without discussing them at first.  If you go with (2), I think you will have two entire subsections with multiple plots but no description of the results, which seems like it will be hard for readers to follow (as you then collect all the interpretation elsewhere).}\tianqing{Restructure the section to 4.1: full analyses,  4.2: a much shorter two parameter cases, 4.3: a short summary of the results.}



%\rachel{Need to say what vertical and horizontal lines are.}\done% \rachel{I think this figure needs some work.  When you have 100 points and lines on top of each other, it is different to impossible to see the transparency of each one (they could just appear dark because two are on top of each other).  I recommend using some color scheme to indicate the weight instead.}\tianqing{I have changed to the best color scheme. I've also make the dots a little transparent so they are more visible.} 

    %\rachel{Caption and figure are inconsistent in use of hats on variables.  Legend should say `Estimate', not `Estimation' (estimation is a process, while the noun `estimate' is the result -- and you are showing the result).}\tianqing{Fixed. I didn't know `estimate' is also a noun, got to love the English intricacies.} \rachel{Pronounced differently:  \url{https://dictionary.cambridge.org/us/pronunciation/english/estimate} (you can play audio for the verb and noun versions).  Yes, English is ridiculous.  I just shared this for information, but feel free to comment this out once you read it.}
    
    
    %\tianqing{What needs to be highlighted in the conclusion
%\begin{itemize}
%    \item We proposed a statistically-principled method, Bayesian resampling
%    \item We explore the $n(z)$ marginalization with the new approach along with the direct resampling and traditional shift model, in a mock analyses for HSC y3 and full dataset. 
%    \item Compare the different approaches. Highlight the results for HSC Y3, that shift model works fine, and is recommended.
%    \item Point out implication for future analyses from the HSC full data analyses: we shouldn't trust direct sampling, shift model's drawback.
%    \item Motivation for future work: fast resampling method (something like importance sampling), to mitigate the intensive computational cost.
%\end{itemize}}

%\rachel{I feel like this is missing an overarching high-level statement to tie everything together, something like `The goal of this work was to understand the performance of methods for incorporating uncertainty in the ensemble redshift distribution in cosmological weak lensing shear analyses, including their impact on computational expense and on the estimated uncertainties on cosmological parameters.'  Diving straight down into Bayesian resampling seems too far into the details.}\tianqing{Agree. I have added your sentence at the begining.}

%\rachel{The conclusions section should focus on your conclusions.  It is unnecessary to mention every single test, if the conclusion of that test was the same as the others.  Therefore, I suggest eliminating this entire paragraph.} \done We conduct a simpler 2-parameter analysis, where only $\Omega_m$ and $\sigma_8$ are set free, as an initial sanity check and software validation test. All aforementioned conclusions still hold for the 2-parameter analyses.

%\rachel{I think that this paragraph needs context: the above-mentioned results were with noise-free data vectors only, and then explain why this test with noisy data vectors is valuable.}\tianqing{Added a high level motivation of doing PIT, and add ` [...], to ensure robustness of our results on the real analysis.'} 



% \section{Comparison between $n(z)$}
% \label{sec:ap:comp}

% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{plot/full_y3_takashi.pdf}
%     \caption{Posterior distribution of $\Omega_m$ - $S_8$ comparison between our $n(z)$ and the stacked $p(z)$. Both cases use shift model, with prior specified correspondingly, and use our noiseless data vector and $\mt{\Sigma}_{\rm y3}$. The stacked $p(z)$ induces a negative bias in $S_8$, which is consistent with the fact that the stacked $p(z)$ has a higher mean redshift than our $n(z)$ distribution in all four bins. }
%     \label{fig:200chains}
% \end{figure}


% We run the full parameter inference with our data vector and covariance $\mt{\Sigma}_{\rm y3}$, but change the redshift distribution and the shift model prior to the values in \cite{2020PASJ...72...16H}. Our $n(z)$ prior has a lower average shift and a narrower prior than the distribution in \cite{2020PASJ...72...16H}. This results in a negative bias on $S_8$ at ~$0.5\sigma$, shown in Fig.~\ref{fig:200chains}. The level of increase in $S_8$ errorbar after marginalizing over the $n(z)$ uncertainties is similar to what is found in this work, as the $n(z)$ prior and covariance for three year analysis are both smaller than \cite{2020PASJ...72...16H}.

%\rachel{Would it be cleaner to swap $S_8$ and $S_8'$, i.e., use $S_8'$ as a meaningless integration variable and use $S_8$ as the upper limit, so you end up with a function of $S_8$?}\tianqing{Right, fixed.}
%\rachel{For those who are not familiar with the PIT theorem, it may be useful to specify that when you say $Y=$\dots, you mean that $Y$ is a random number drawn from that distribution (or at least I think so?  if I'm wrong, perhaps that emphasizes the importance of saying what $Y$ is and why you need a new symbol there, in addition to defining $F_{S_8}(S_8')$}\tianqing{You are right, $Y$ is a random variable. I have added a bit more explanation in the next sentence.} \rachel{I personally find this equation confusing, as $F_{S_8}(S_8)$ appears to be a function, and you are now assigning $Y$ to be equal to that function.  I don't think it's standard to use $=$ to mean `is a random variable drawn from this distribution'.  So I would suggest eliminating the $Y=$ from equation 18 (which works better with the start of the sentence beforehand, since it claims the purpose of equation 18 is to define the CDF).  Then in the sentence afterwards you say $Y$ is a random variable that we will draw from this CDF, and that becomes the definition of $Y$.}\tianqing{Yes, I think that make sense. Fixed.}






% In this subsection we briefly describe the basic methodology employed in this work for inferring ensemble redshift distributions. The methodology is an extension of the work in \citet{2022MNRAS.509.4886R} that will be described in more detail in another paper (Rau et al. {\em in prep}). We therefore focus in this section on a brief methodological description. We split the discussion into three parts: a description of the inference methodology that utilizes the redshift information in the galaxies' photometry (\S~\ref{subsec:inference_photometry}), which includes a treatment of model uncertainty. In \S~\ref{subsec:meas_z_dependent_dm} we discuss the measurement of the redshift-dependent galaxy-dark matter bias in the CAMIRA LRG sample~\citep{Oguri2014, Oguri2017a, Oguri2017b}, %\rachel{reference needed}\ben{Added.}, 

% which is an important modelling component of the spatial cross-correlation data vector. In \S~\ref{subsec:joint_inference_camira} we then discuss our joint inference methodology that combines redshift information from both the photometry of galaxies and the spatial cross-correlations with the CAMIRA LRG sample. Throughout this subsection we will refer to the appendices for the technical details and more in-depth considerations.  %\ben{Maybe put this above into (2), or push 2.2-4 one level down to subsubsections. Giving an overview on the same hierarchical level as the following subsections could be confusing.}\tianqing{I suggest turning Section 2.1 - 2.4 into section 2.1, with 3 subsubsections.}

% \subsubsection{Inference using Photometric Data}
% \label{subsec:inference_photometry}
% %\rachel{This subsubsection has no references until it's nearly over, and that's for a technical detail.  I strongly recommend opening this with a high-level explanation of where this method is coming from, with appropriate references.  This is important context (otherwise it almost sounds like you're describing a completely new method that happens to refer to Rau et al 2021 for one detail).}
% %% What's below is now less important because the same thing is said above this subsubsection.
% %The sample redshift distribution posteriors that we use in this publication are constrained using both the broadband photometry of galaxies as well as the spatial cross-correlations of the photometric sample with the CAMIRA LRG sample. The methodology used to construct these posteriors is an extension of the work described in  \citet{2022MNRAS.509.4886R} and will, as mentioned previously, described in more detail in Rau, et al. {\em (in prep)}.  

% Denoting the set of photometry measurements as $F := \{f_i | i \in (1, ..., N_{\rm gal}\}$ we can describe the forward model that generates the data as a draw from a sample redshift distribution $p(z | \mathbf{nz})$, where $\mathbf{nz}$ denotes a set of parameters that describes the sample redshift distribution, and $N_{\rm gal}$ denotes the galaxy sample size. %\ben{Maybe define $N_{\mathrm{gal}}$ here where it's first used (currently defined further down).}\done 
% The redshift $z$ of the galaxy is then connected with the SED model to yield the galaxies' flux $f$. Describing the measurement process using the flux likelihood $ p(\mathbf{f}_i | \mathcal{T}(z_i), \Sigma)$, where ($\mathcal{T}$, $\Sigma$) denotes the (template model, flux measurement covariance), we can obtain a log-likelihood as: 
% \begin{equation}
%     l(\mathbf{\hat{F}}|\mathbf{nz}) = \sum_{i = 1}^{N_{\rm _{gal}}} \log{\left( \int \mathrm{d}z_i p_{\rm i}(\mathbf{f}_i | \mathcal{T}(z_i), \Sigma_i) \,  p(z_i | \mathbf{nz})\right)} \, .
%     \label{eq:likelihood}
% \end{equation}
% While model uncertainty can in principle be included by adding parameters to the template model, or modifying the likelihood, in practice it can be difficult to devise such a meta-model that captures the different model assumptions. We therefore include model uncertainty in a hierarchical manner by using a joint distribution over the parameters $\mathbf{nz}$ parametrized by $\boldsymbol{\alpha}$. 

% The posterior for this parameter vector $\boldsymbol{\alpha}$ then reads: 
% \begin{equation}
%     p(\boldsymbol{\alpha} | \mathbf{nz}, \mathcal{M}) \propto \prod_{\mathcal{M}} \left( \prod_{\rm j=1}^{N_{\rm gal}} \int dz_j p_j^{\mathcal{M}}(z_j) p(z_j | \mathbf{nz}_{\mathcal{M}}) \right) p\left(\mathbf{nz}_{\rm \mathcal{M}} | \boldsymbol{\alpha}\right) \, .
%     \label{eq:def_posterior}
% \end{equation}

% Here we abbreviated the likelihoods of the individual models as $ p_j^{\mathcal{M}}(z_j)$. For consistency with the literature we will call these functions `individual galaxy redshift distributions' in the following. 

% We note however that this term is not precisely defined in the literature, as it refers to both likelihoods of forward models and conditional probability density functions obtained in a regression setting. These are very different statistical quantities that are comparable only if the implicit priors in the latter can be neglected. Eq.~\eqref{eq:def_posterior}. Our model set consists of a template fitting code `Mizuki' that defines a likelihood, empirical codes `MLZ', `Ephor' that would define a conditional probability density function obtained on a training set and  `FrankenZ' that uses a flux-error weighted score function to map training set objects to galaxies in the photometric dataset. We refer to \citet{2018PASJ...70S...9T} for a summary of the different methodologies that are available to us. 

% Since the forward model of our estimation strategy connects a true unknown sample redshift distribution to a measured flux, the estimation of the formed is an example for an inverse problem that requires a regularization strategy to supress spurious noise in the estimate.

% Following \citet{10.1093/mnras/stab3290} we use regularizing functionals to induce smoothness of the sample redshift distribution while avoiding undercoverage of credibility intervals. We use the set of simple trapezoid integral within a coarser grid to `smooth' the sample redshift distribution estimate
% \begin{equation}
%     \mathcal{F} := \{(z_R - z_L) (nz_L + nz_R) | (z_L, z_R) \in \mathcal{I}(h)\} \, ,
%     \label{eq:reg_functional}
% \end{equation}
% where $\mathcal{I}$ denotes the set of intervals on the grid that depends on the number of bins $h$. The variables $nz_{L/R}$ denotes the (left/right) bin edges. By sampling from Eq.~\eqref{eq:def_posterior} we can then fit a Dirichlet distribution on the larger grid to obtain a posterior for the regularized bins $p(\boldsymbol{\alpha}_{\rm Reg} | \mathbf{nz}_{\rm Reg}, \mathcal{M})$. We fit $h$ jointly with the cross-correlation data vector described in the following section.

% \subsubsection{Measurement of redshift dependent Galaxy-Dark Matter bias}
% \label{subsec:meas_z_dependent_dm}
% We measure the redshift dependent galaxy-dark matter bias function of the CAMIRA LRG survey in annular bins from $1.5 - 5.0$ Mpc. We assume a $\Lambda$-CDM cosmology for the $\xi_{\rm DM}$ prediction with 
% $\Omega_{\rm CDM} = 0.259$, $\Omega_b = 0.048$, $h = 0.678$, $n_s = 0.95$ and $\sigma_8 = 0.8$, following \citet{2016A&A...594A..13P}. \ben{Maybe justify the parameters with a citation or two, like Planck+2015 for the $h$ value.}\tianqing{I have cited the Planck+2015 results here, but need confirmation from Markus.} We note that the bias measurements are relatively insensitive against changes in cosmology given the current signal to noise. We use the sample redshift distribution of the CAMIRA LRG sample determined using the photometric redshifts to determine the redshift dependent bias shown in Fig.~\ref{fig:bias_model_camira}. \markus{We show the resulting redshift dependent galaxy-dark matter posteriors based on the log-likelihood constructed using measurements of the CAMIRA-LRG self correlations. The diagonal covariance of the aforementioned likelihood is constructed using bootstrap resampling.} The blue horizontal lines show the corresponding measurements from \citet{2021arXiv210308628I}. The red span corresponds to the $\pm 1\sigma$ posterior of the linear bias fit $b(z) = b_0(1+z)$. We see that our measurements are consistent with  \citet{2021arXiv210308628I} within the error. The excess signal at $z \approx 0.4$ could be indicative of a population of catastrophic outliers. These outlier mismatches between galaxies at $z < 0.5$ and $z \leq 2.5$ can be induced by lyman-balmer break confusion. However the signal is not significant compared with the errorbar and the results from the template fitting analysis does not indicate a strong population of redshift outliers at this redshift. We, therefore, find the explanation of this feature inconclusive. Since this excess signal will not change the methodology and conclusions of this work, we refer to a follow-up analysis in the upcoming S19A data release. 

% %\rachel{In the caption of figure 1, I raised some methodology questions here, but I want to flag for the text that there are some questions that are not answered in either the text or caption, such as how the errorbars are determined.}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.35]{Biasmodel.png}
%     \caption{Redshift dependent galaxy-dark matter bias of the CAMIRA LRG sample within scales of 1.5-5 Mpc.The blue horizonal curves show the galaxy-dark matter bias measurements from \citet{2021arXiv210308628I} and the red contours show the $\pm 1\sigma$ error on a linear redshift dependent galaxy-dark matter bias model fit. The errrorbars show $\pm 1 \sigma$ errorbars. \markus{The covariance matrix of the cross-correlation measurements that are used to construct these posteriors are constructed using bootstrap resampling.}  with a covariance matrix boot. %\rachel{Plot needs a horizontal axis label.  Vertical axis label is kind of cut off so I can't quite tell what it says - should work on this.  Also, what is the rationale to use $\xi$ (3D) rather than a projected correlation, especially given uncertainties in the CAMIRA photo-z?  Also on these scales, $\xi$ will suffer from FoG and other effects that are difficult to model.}
%     }
%     \label{fig:bias_model_camira}
% \end{figure}

% \subsubsection{Joint Inference with Spatial Cross-Correlations with CAMIRA}
% \label{subsec:joint_inference_camira}
% In the previous two subsections we discussed our model combination scheme and our measurement of the redshift dependent galaxy-dark matter bias. Here we put these components together in a joint likelihood of both spatial cross-correlations between the HSC-S16A sample with the CAMIRA-LRG sample and the model combined likelihood constructed using the photometric redshift estimates. 
% The spatial cross-correlation between the Camira-LRG (c) sample and photometric sample (p) can be predicted as 
% \begin{equation}
%     \mathbf{w_{\rm sc}} \propto \mathbf{nz}_p \, \mathbf{b_p} \,  \mathbf{b_c}  \, \mathbf{w_{\rm DM}} \, , 
%     \label{eq:wx_definition}
% \end{equation}
% where $w_{\rm DM}$ is the scale averaged, redshift and cosmology dependent, two point function of the dark matter density field. The terms $b_s$ and $b_c$ are redshift dependent galaxy-dark matter bias terms and $nz_p$ are the sample redshift distribution of the HSC photometric sample to be estimated. We use `The-Wizz' \citep{2017MNRAS.467.3576M} to measure these cross-correlations and bootstrap resampled error estimates. For the measurements we choose a scale annulus of $1.5-5.0 \, {\rm Mpc}$ in analogy to \citet{2020arXiv201208569G}.

% As described in detail in \S~6 in \citet{10.1093/mnras/stab3290}, the posterior of parameters that describe the redshift distribution $\mathbf{nz}$ are then given by the product of this cross-correlation likelihood and the photometric likelihood.

% Here we extend this model by fitting a Dirichlet prior with parameters informed by the model set $\mathcal{M}$ as explained in \S~\ref{subsec:inference_photometry}. As detailed in \S~\ref{sec:derivation_inference_scheme} we use an empirical bayes scheme to fit the parameter $\boldsymbol{\hat{\alpha}_{\rm Reg}}$ using an empirical bayes scheme that is then regularized using the procedure described in the previous section. We reiterate that the parameter $h$ that governs the smoothing is jointly fitted with the cross-correlation data vector. 

% The posterior informed by both the cross-correlation data vector $w_{\rm meas}$ and the posterior of sample redshift distribution parameters that include model error as defined in the previous section $p(\mathbf{nz} | \boldsymbol{\hat{\alpha}_{\rm Reg}}, \mathbf{pz})$ are then given as 
% \begin{equation}
%   p(\mathbf{nz} | \mathbf{w_{\rm meas}}, \boldsymbol{\hat{\alpha}_{\rm Reg}}, \mathbf{pz}) \propto  p(\mathbf{w}_{\rm meas} | w(\mathbf{b_p}, \mathbf{b_C}), \boldsymbol{\Sigma}) p(\mathbf{nz} | \boldsymbol{\hat{\alpha}_{\rm Reg}}, \mathbf{pz}) \, .
%   \label{eq:posterior_joint}
% \end{equation}
% For ease of notation we abbreviated here the set of individual galaxy redshift distributions from the different models as $\mathbf{pz}$.

% The parameters $\mathbf{b_c}$ that describes the redshift dependent galaxy-dark matter bias using the auto-correlation of the Camira sample as discussed in \S~\ref{subsec:meas_z_dependent_dm}. We assume a constant galaxy-dark matter bias of the photometric sample $b_p$ and absorb it into the normalization factor of the sample redshift distribution of the HSC S16A sample in the inference. We sample the posterior defined in Eq.~\eqref{eq:posterior_joint} using the Self-Adjusting Logit Transform (SALT) sampler \citep{doi:10.1080/00949655.2017.1376063}. The proposal distribution of the SALT sampler is designed to efficiently traverse parameters that describe the amplitude of histogram bins of probability density functions. A primary complication in these cases is that these parameters have to sum to unity which requires a custom proposal distribution. 

% Both the normalization factor of the sample redshift distribution and the parameters $\mathbf{b}_c$ are well constrained and will not induce large differences in the posterior, so we fix them to their maximum likelihood value for simplicity. Assuming a linear relation of the redshift dependent galaxy-dark matter bias of the CAMIRA-LRG sample of the form $b(z) = b_c (1 + z)$, the maximum likelihood value using the autocorrelation measurements is given to be $b_{\rm c, ML} = 1.06$. As noted earlier we optimize for the grid resolution $h$ defined in Eq.~\eqref{eq:reg_functional}. 


















